The Relationship Between Molecular Gas, HI, and Star Formation in the Low-Mass, Low-Metallicity Magellanic Clouds

The Magellanic Clouds provide the only laboratory to study the effect of metallicity and galaxy mass on molecular gas and star formation at high (~20 pc) resolution. We use the dust emission from HERITAGE Herschel data to map the molecular gas in the Magellanic Clouds, avoiding the known biases of CO emission as a tracer of H$_{2}$. Using our dust-based molecular gas estimates, we find molecular gas depletion times of ~0.4 Gyr in the LMC and ~0.6 SMC at 1 kpc scales. These depletion times fall within the range found for normal disk galaxies, but are shorter than the average value, which could be due to recent bursts in star formation. We find no evidence for a strong intrinsic dependence of the molecular gas depletion time on metallicity. We study the relationship between gas and star formation rate across a range in size scales from 20 pc to ~1 kpc, including how the scatter in molecular gas depletion time changes with size scale, and discuss the physical mechanisms driving the relationships. We compare the metallicity-dependent star formation models of Ostriker, McKee, and Leroy (2010) and Krumholz (2013) to our observations and find that they both predict the trend in the data, suggesting that the inclusion of a diffuse neutral medium is important at lower metallicity.

==> table1.tex <==
%% This is file `LMC_SF_table1.tex',
\ProvidesFile{MC_SF_table1.tex}
%
\begin{deluxetable*}{ccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablecaption{Total Molecular Gas Mass Estimates for the LMC and SMC \label{table:compare_H2}}
\tablehead{\colhead{ } & \colhead{Data} & \colhead{Dust Fitting\tablenotemark{a}} & \colhead{Method} & \colhead{\Mmol\ [$10^{7}$\msol]\tablenotemark{b}}} 
\startdata
\multicolumn{5}{c}{\textbf{LMC}} \\
1&$Herschel$ 100-350\micron&MBB, $\beta=1.8$&\dGDR\ map\tablenotemark{c}&9.9\\
2&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}&6.3\\
3&$Herschel$ 100-350\micron&MBB, $\beta=1.5$&\dGDR\ map\tablenotemark{c}&6.8\\
4&$Herschel$ 100-350\micron&MBB, $\beta=2.0$&\dGDR\ map\tablenotemark{c}&10.1\\
5&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}, no \hi\ offset&13.4\\
6&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&GDR $=540$\tablenotemark{d}&3.9\\
7&$Herschel$ 100-350\micron&MBB, $\beta=1.8$&\dGDR\ map\tablenotemark{c}, $\delta_{\textnormal{GDR,dense}}=0.5\delta_{\textnormal{GDR,map}}$&4.5\\
8&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}, $\delta_{\textnormal{GDR,dense}}=0.5\delta_{\textnormal{GDR,map}}$&4.0\\
\\
\multicolumn{5}{c}{\textbf{SMC}} \\
9&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}&2.0
\enddata
\tablenotetext{a}{MBB = Modified Black Body, BEMBB = Broken Emissivity Modified Black Body}
\tablenotetext{b}{assuming $d_\textnormal{LMC}=50$ kpc and $d_\textnormal{SMC}=62$ kpc}
\tablenotetext{c}{map of spatially varying \dGDR, see Section \ref{subsection:h2_method}}
\tablenotetext{d}{does not include factor of 1.36 contribution from helium}
\label{table:h2_maps}
\end{deluxetable*}
\endinput

==> table2.tex <==
%% This is file `LMC_SF_table2.tex',
\ProvidesFile{LMC_SF_table2.tex}
%
\begin{center}
\begin{deluxetable}{ccc}
\tablecolumns{3}
\tablewidth{0pc}
\tablecaption{Global Properties \label{table:global_properties}}
\tablehead{\colhead{Property} & \colhead{LMC} & \colhead{SMC}} 
\startdata
$M^{\textnormal{dust}}_{\textnormal{mol}}$ & $6.3^{+6.3}_{-3.2} \times 10^{7}$ \msol & $2.0^{+2.0}_{-1.0} \times 10^{7}$ \msol \\
$L_{\textnormal{CO}}$ & $7\times10^{6}$ K km s$^{-1}$\tablenotemark{a} & $1.7\times10^{5}$ K km s$^{-1}$\tablenotemark{b} \\
\Mhi & $4.8 \times 10^{8}~\msol$\tablenotemark{c} &  $3.8 \times 10^{8}~\msol$\tablenotemark{d} \\
\Mstar & $2\times10^{9}~\msol$\tablenotemark{e} & $3\times10^{8}~\msol$\tablenotemark{f} \\
SFR\tablenotemark{d} & 0.20 \msol\ yr$^{-1}$  & 0.033 \msol\ yr$^{-1}$ \\
\taumoldep & $0.37^{+0.37}_{-0.19}$ Gyr & $0.61^{+0.61}_{-0.31}$ Gyr
\enddata
\tablenotetext{a}{\citet{fuk08}, no sensitivity cuts}
\tablenotetext{b}{\citet{miz01}, no sensitivity cuts}
\tablenotetext{c}{\citet{sta03}}
\tablenotetext{d}{\citet{sta99}}
\tablenotetext{e}{\citet{ski12}}
\tablenotetext{f}{assuming $A_{V}(\text{LMC})=0.2$ mag and $A_{V}(\text{SMC})=0.1$ mag}
\label{table:integrated_properties}
\end{deluxetable}
\end{center}
\endinput

==> table3.tex <==
%% This is file `LMC_SF_table3.tex',
\ProvidesFile{MC_SF_table3.tex}
%
\begin{deluxetable*}{cccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pc}
\tablecaption{Comparison of Total Molecular Gas Mass Estimates for the LMC and SMC \label{table:compare_H2}}
\tablehead{\colhead{ } & \colhead{Data} & \colhead{Dust Fitting\tablenotemark{a}} & \colhead{Method} & \colhead{\Mmol\ [$10^{7}$\msol]\tablenotemark{b}} & \colhead{Reference} } 
\startdata
\multicolumn{6}{c}{\textbf{LMC, this work}} \\
1&$Herschel$ 100-350\micron&MBB, $\beta=1.8$&\dGDR\ map\tablenotemark{c}&9.9&1\\
2&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}&6.3&1\\
3&$Herschel$ 100-350\micron&MBB, $\beta=1.5$&\dGDR\ map\tablenotemark{c}&6.8&1\\
4&$Herschel$ 100-350\micron&MBB, $\beta=2.0$&\dGDR\ map\tablenotemark{c}&10.1&1\\
5&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}, no \hi\ offset&13.4&1\\
6&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&GDR $=380$\tablenotemark{d}&1.1&1\\
7&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&GDR $=540$\tablenotemark{d}&3.9&1\\
8&$Herschel$ 100-350\micron&MBB, $\beta=1.8$&\dGDR\ map\tablenotemark{c}, $\delta_{\textnormal{GDR,dense}}=0.5\delta_{\textnormal{GDR,map}}$&4.5&1\\
9&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}, $\delta_{\textnormal{GDR,dense}}=0.5\delta_{\textnormal{GDR,map}}$&4.0&1\\
10&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&GDR$_{\text{diffuse}}=540$, GDR$_{\text{dense}}=330$\tablenotemark{d}&2.2&1\\
\\
\multicolumn{6}{c}{\textbf{LMC, literature}} \\
11&$Herschel$ 100-500\micron,&BEMBB, $0.8<\beta<2.5$&GDR$_\text{diffuse}=380$, $X_\text{CO}=2\times10^{20}$&2.7&2\\
&MAGMA \co&&&\\
12&$IRIS$, $Spitzer$ 3-160\micron&\citet{des90}&lowest 5\% \dGDR&33&3\\
13&$IRAS$ 12-100\micron&\nodata& reference $N_{\text{H}}/\mu_{\textnormal{FIR}}$&15.4&4\\
14&NANTEN \co&\nodata&Galactic $\alpha_{\textnormal{CO}} = 4.3$&1.25&5\\
15&NANTEN \co&\nodata&$X_{\textnormal{CO}} = 7\times10^{20}$&5&5\\
\\
\multicolumn{6}{c}{\textbf{SMC, this work}} \\
16&$Herschel$ 100-500\micron&BEMBB, $0.8<\beta<2.5$&\dGDR\ map\tablenotemark{c}&2.0&1\\
\\
\multicolumn{6}{c}{\textbf{SMC, literature}} \\
17&$Herschel$ 100-500\micron,&BEMBB, $0.8<\beta<2.5$&GDR$_\text{diffuse}=1200$, $X_\text{CO}=1\times10^{21}$&0.2&2\\
&NANTEN \co&&&\\
18&$Spitzer$ 70-160\micron&MBB, $\beta=1.5$&\dGDR\ map\tablenotemark{c}&2.2&6\\
19&$IRIS$ 100,$Spitzer$ 160\micron&\citet{dal02}&regional GDR&3.2&7\\
20&$IRAS$ 12-100\micron&\nodata&reference $N_{\text{H}}/\mu_{\textnormal{FIR}}$&10.5&4\\
21&NANTEN \co&\nodata&Galactic $\alpha_{\textnormal{CO}} = 4.3$&0.07&8\\
22&NANTEN \co&\nodata&$X_{\textnormal{CO}} = 2.5\times10^{21}$&0.42&8
\enddata
\tablerefs{(1) this work, (2) \citet{rom14}, (3) \citet{ber08}, (4) \citet{isr97}, (5) \citet{fuk08}, (6) \citet{bol11}, (7) \citet{ler07}, (8) \citet{miz01}}
\tablenotetext{a}{MBB = Modified Black Body, BEMBB = Broken Emissivity Modified Black Body}
\tablenotetext{b}{assuming $d_\textnormal{LMC}=50$ kpc and $d_\textnormal{SMC}=62$ kpc}
\tablenotetext{c}{map of spatially varying \dGDR, see Section \ref{subsection:h2_method}}
\tablenotetext{d}{does not include factor of 1.36 contribution from helium}
\label{table:h2_estimates}
\end{deluxetable*}
\endinput
